Learning Min-norm Stabilizing Control Laws for Systems with Unknown Dynamics

This paper introduces a framework for learning a minimum-norm stabilizing controller for a system with unknown dynamics using model-free policy optimization methods. The approach begins by first designing a Control Lyapunov Function (CLF) for a (possibly inaccurate) dynamics model for the system, along with a function which specifies a minimum acceptable rate of energy dissipation for the CLF at different points in the state-space. Treating the energy dissipation condition as a constraint on the desired closed-loop behavior of the real-world system, we use penalty methods to formulate an unconstrained optimization problem over the parameters of a learned controller, which can be solved using model-free policy optimization algorithms using data collected from the plant. We discuss when the optimization learns a stabilizing controller for the real world system and derive conditions on the structure of the learned controller which ensure that the optimization is strongly convex, meaning the globally optimal solution can be found reliably. We validate the approach in simulation, first for a double pendulum, and then generalize the framework to learn stable walking controllers for underactuated bipedal robots using the Hybrid Zero Dynamics framework. By encoding a large amount of structure into the learning problem, we are able to learn stabilizing controllers for both systems with only minutes or even seconds of training data.

==> io_linearization.tex <==
% However, designing CLF candidates for complex systems is in general a difficult problem, which constitutes a current area of research (\todo{put in a citation, maybe Packard's paper?}. Fortunately, for input-output linearizable systems we can follow a systematic approach to design CLF candidates by defining the CLFs on the input-output linearized dynamics of the system, as done in (\todo{put in a citation}. In this section we will revisit this systematic approach to CLF design and adapt the learning problem \eqref{eq:clf_opt} to the case of CLFs that are defined on the input-output linearized dynamics of the system.

% \subsection{Input-Output Linearization}
% Let's define $y_p \in \R^m$ as the set of outputs of the plant \eqref{eq:plant}
% \begin{equation}
% \label{eq:system_io}
%     \begin{aligned}
%         &\dot{x}_p=f_p(x_p)+g_p(x_p)u_p,\\
%         &y_p=h_p(x_p).
%     \end{aligned}
% \end{equation}

% \begin{assumption}\vspace{0.3cm}\label{ass:relative_degree_stuff}
% The vector relative degree of the outputs $y_p$ is well-defined and its value is $\gamma$.
% \vspace{0.3cm}
% \end{assumption}

% Then, we can write

% \begin{equation}
% y^{(\gamma)}_p=L_{f_p}^{\gamma} h_p(x_p)+L_{g_p} L_{f_p}^{\gamma-1} h_p(x_p) u_p, \label{eq:2}
% \end{equation}

% \noindent where the functions $L_{f_p}^{\gamma}h_p$ and $L_{g_p}L^{\gamma-1}_{f_p}h_p$ are the $\gamma^{th}$ order Lie derivatives of the outputs. And from Assumption \ref{ass:relative_degree_stuff} we have that $L_{g_p} L_{f_p}^{\gamma-1} h_p(x_p) \not= 0$ $\forall x_p\in D$, with $D\subset \mathbb{R}^{n}$ being a compact subset of the state space which contains the origin. The control input law

% \begin{equation} \label{eq:io_lin_input}
%     u_p(x_p)=L_{g_p} L_{f_p}^{\gamma-1} h_p(x_p)(-L_{f_p}^{\gamma}h_p +\mu)
% \end{equation}

% \noindent renders the input-output dynamics of the system linear $y^{(\gamma)}_p = \mu$, where $\mu$ is an additional input that is typically designed to be a feedback on the outputs $y_p$. A system of the form \eqref{eq:system_io} that satisfies Assumption \ref{ass:relative_degree_stuff} is consequently said to be input-output linearizable.

% Using the state transformation $\Phi : x_p \rightarrow (\eta_p, z_p)$, with the transverse dynamics defined as
% \begin{equation}
% \eta_p =[h_p(x_p)^{\top},L_{f_p}h_p(x_p)^{\top},...,L_{f_p}^{\gamma-1} h_p(x_p)^{\top}]^{\top},
% \end{equation}
% and $z_p \in Z_p$, where $ Z_p=\{ x_p \in \mathbb{R}^{n} |\ \eta_p = 0\}$, the closed-loop dynamics of the system become

%  \begin{equation}
%  \left\lbrace
%       \begin{aligned}
%          \dot{\eta_p} & = F\eta_p +G\mu,\\
%          \dot{z}_p & = \psi_p(\eta_p,z_p),
%       \end{aligned}
%     \right.
%     \label{eq:linear-dynamics}
% \end{equation}
% being a linear time-invariant (LTI) system on the transverse dynamics $\eta_p$ with $F\in \R^{m\gamma\times m\gamma}$ and $G\in \R^{m\gamma\times m}$
% \begin{equation}
% F=\left[\begin{array}{ccccc}
% {0} & {I_m} & {.} & {.} & {0} \\
% {0} & {0} & {I_m} & {.} & {0} \\
% {.} & {.} & {.} & {} & {} \\
% {0} & {.} & {.} & {.} & {I_m} \\
% {0} & {.} & {.} & {.} & {0}
% \end{array}\right] \text { and } G=\left[\begin{array}{l}
% {0} \\
% {.} \\
% {.} \\
% {0} \\
% {I_m}
% \end{array}\right],
% \end{equation}
% and the zero-dynamics on $z_p$.
% \subsection{Input-Output Linearized Dynamics CLF-based Control} \label{subsec:clfs}

% We can now define the control input $\mu$ as a feedback law on $\eta_p$: $\mu =  K\eta_p$, with $K\in\R^{m\times m\gamma}$ and design it such that the transverse dynamics become exponentially stable. This yields the closed-loop LTI system on the transverse dynamics $\dot{\eta_p} = A_{cl}\eta_p$, with $A_{cl} = F + GK$.

% It is now straight forward to choose a quadratic CLF candidate on the linear transverse dynamics of the system \eqref{eq:linear-dynamics}
% \begin{equation}
%   V(\eta_p)=\eta_p^{T} P \eta_p,
% \end{equation}
% where $P$ is the solution of the Lyapunov Equation $A_{cl}^{T}P + P A_{cl} = -Q$, and Q can be any symmetric positive-definite matrix.

% Now that we have a CLF candidate, we can apply the reasoning of Sections \ref{subsec:clfs} and \ref{subsec:learn-min-norm} to the transverse dynamics defined by the first equation of \eqref{eq:linear-dynamics}. This yields the control law that is defined point-wise by
% \begin{align}
%     \mu^*(\eta_p) & = \argmin_{\mu \in \R^m} \norm{\mu}_2^2 \\ 
%     & \text{s.t.}  \ \nabla V(\eta_p)[F\eta_p + G\mu] \leq -\sigma(\eta_p).
%     \vspace{0.3cm}
% \end{align}
% Then, following equation \eqref{eq:io_lin_input}, the input-output linearizing controller that stabilizes the transverse dynamics of the plant is given by
% \begin{equation} \label{eq:io_lin_input_opt}
%     u_p^*(x_p)=L_{g_p} L_{f_p}^{\gamma-1} h_p(x_p)(-L_{f_p}^{\gamma}h_p +\mu^*(x_p))
% \end{equation}

% \subsection{Learning a Min-norm Transverse Dynamics Stabilizing Controller} \label{subsec:learn-min-norm-iolin}
% However, the expression of the input-output linearizing controller \eqref{eq:io_lin_input_opt} depends heavily on the dynamics of the plant and, therefore, if they are unknown we cannot compute the value of $u_p^*(x_p)$ directly. We now need to adapt the reasoning of Section \ref{subsec:learn-min-norm} to the method of designing CLFs on the input-output linearized dynamics of the system that has just been presented.

% We will again use the nominal model of \eqref{eq:nominal_dynamics} and define a set of outputs $y_m$



